Modeling Bilateral Lymphatic Head and Neck Tumour Progression for Personalized Elective Target Volume Definition

Objective: Large irradiated volumes are a major contributor to severe side-effects in patients with head and neck cancer undergoing curatively intended radiotherapy. We propose a data-driven approach for defining the elective clinical target volume (CTV-E) on a patient-specific basis, with the potential to reduce irradiated volumes compared to standard guidelines. Approach: We introduce a bilateral Bayesian Network (BN), trained on a large cohort, to estimate the patient-specific risk of undetected nodal involvement for both ipsilateral and contralateral lymph node levels (LNLs) I, II, III, and IV, using clinical features, such as patterns of nodal involvement, T-stage, tumour location. By applying risk thresholds, we generated individualized, risk-dependent CTV-E's for representative patient scenarios and compared the resulting treatment volumes and residual risk to those recommended by standard clinical guidelines. Main results: We computed the risks for a set of representative patient scenarios including 1) N0 (T1 and T2 tumour stage), 2) N+ in ipsilateral LNL II (T1 and T2 tumour stage), 3) N+ in ipsilateral LNL II and III (T1 and T2 tumour stage), and 4) N+ of both ipsilateral and contralateral LNL II (T3 and T4 tumour stage). Depending on the chosen risk threshold, the bilateral BN allowed for reductions in irradiated volumes relative to standard clinical protocols. For every patient scenario considered, the CTV-E's defined by the applied risk thresholds were associated with a low estimated probability of undetected nodal involvement in any excluded LNL. Significance: We present a data-driven framework for personalized CTV-E definition, encouraging the discussion of more patient-specific elective nodal target volumes, with potential for de-escalation of irradiated elective volumes.

==> Notes_For_My_Thoughts/Notes.tex <==
\section{Parameter Learning}

The probabilistic structure of the bilateral Bayesian network is governed by a set of parameters \(\theta = \{t_{p \to v}, b_v\}\), where \(t_{p \to v}\) denotes the probability of microscopic tumor spread from lymph node level \(p\) to level \(v\), and \(b_v\) is the baseline probability of direct spread from the primary tumor to level \(v\). These parameters define the conditional probability tables \(P(x_\ell^s \mid \text{Pa}(x_\ell^s))\) used in the generative model described in the previous section.

To estimate \(\theta\), we uses a Bayesian framework. Let \(\mathcal{D} = \{\mathbf{y}_{1}, \dots, \mathbf{y}_{K}\}\) denote the set of unique observed nodal involvement patterns in a cohort of patients, where each \(\mathbf{y}^{(i)}\) is a binary vector encoding radiological findings across lymph node levels and sides. Let \(f_i\) be the frequency of pattern \(\mathbf{y}^{(i)}\) in the dataset. These observed variables are noisy indicators of the latent states \(\mathbf{x}\), which must be integrated out. Using Bayes’ rule, the posterior distribution over parameters given the observed data is:

\begin{equation} \label{eq:Bayes}
P(\theta \mid \mathcal{D}) = \frac{P(\mathcal{D} \mid \theta) \, P(\theta)}{\int P(\mathcal{D} \mid \theta') \, P(\theta') \, d\theta'} \tag{1}
\end{equation}

To reflect the probabilistic nature of the parameters, we constrain \(\theta\) to lie within the probability simplex \(\mathcal{S}^{V-1}\), defined by:

\[
\theta \in \mathcal{S}^{V-1} \quad \Leftrightarrow \quad t_{p \to v} \in [0, 1] \quad \text{and} \quad \sum_v t_{p \to v} = 1 \quad \forall \ p.
\]

Under this constraint, we adopt a uniform prior over the admissible region, placing equal weight on all valid configurations:

\[
P(\theta) \propto \mathbb{I}_{\mathcal{S}^{V-1}}(\theta)
\]

where \(\mathbb{I}_{\mathcal{S}^{V-1}}(\theta)\) is the indicator function that equals 1 if \(\theta\) satisfies the simplex constraints and 0 otherwise. The likelihood of each observed pattern \(\mathbf{y}_i\) under parameters \(\theta\) is given by:

\begin{equation}
P(\mathbf{y}_{i} \mid \theta) = \sum_{\mathbf{x}} P(\mathbf{y}_{i} \mid \mathbf{x}) \cdot P(\mathbf{x} \mid T, \theta) \tag{2}
\end{equation}

and the total likelihood over the dataset is given by:

\begin{equation}
P(\mathcal{D} \mid \theta) = \prod_{i=1}^K P(\mathbf{y}_{i} \mid \theta)^{f_i} \tag{3}
\end{equation}

Due to the combinatorial complexity of the latent space, the integral in equation \ref{eq:Bayes} cannot be evaluated exactly due to the high dimensionality of the latent space. Therefore, we estimate the parameters \(\theta\) using Markov chain Monte Carlo (MCMC) sampling, which allows us to approximate the posterior distribution \(P(\theta \mid \mathcal{D})\) without requiring analytic integration. At each iteration, new proposals for \(\theta\) are drawn within the constrained space \(\mathcal{S}^{V-1}\), and their likelihood is computed by marginalizing over latent microscopic states

\subsection{Sampling with Markov Chain Monte Carlo}

In general, modeling conditional probabilities for binary variables in a Bayesian network requires a number of parameters exponential in the number of parents. Specifically, a node with \( N \) binary parents would need \( 2^N \) entries in its conditional probability table to fully specify its distribution. However, we employ a \emph{noisy-OR} formulation to model lymphatic spread, which assumes that each parent contributes independently and additively to the activation of a child node.

Under this assumption, the probability that a lymph node level \( x_\ell^s \) remains uninvolved, given that its parents \( \text{Pa}(x_\ell^s) = \{x_j\} \) are active, factorizes as:
\begin{equation}
P(x_\ell^s = 0 \mid \{x_j = 1\}) = \prod_{j \in \text{Pa}(x_\ell^s)} (1 - p_{j \rightarrow \ell})
\end{equation}
where \( p_{j \rightarrow \ell} \) denotes the probability that involvement at node \( j \) causes involvement at node \( \ell \). Thus, only one parameter per parent-child edge is required, reducing the complexity from exponential to linear in the number of parents.

In our bilateral model, each side consists of four LNLs (I–IV), with anatomical progression encoded by directed arcs and direct influence from the primary tumor. This structure yields seven parameters per side. Consequently, the full bilateral model comprises only 14 parameters, a substantial reduction compared to the \(2^N\)-sized CPTs required under a general formulation. This compact representation allows for efficient posterior inference from limited data.

To estimate the posterior distribution over model parameters, we used the Python package emcee, which implements an affine-invariant Markov chain Monte Carlo (MCMC) ensemble sampler. This approach is particularly well suited for exploring constrained, correlated parameter spaces such as the probability simplex in our model.

Despite its computational cost, MCMC sampling remains one of the most robust and flexible methods for posterior inference, especially in models where latent variables must be marginalized numerically. In our study, sampling exhibited favorable convergence properties, with autocorrelation times typically on the order of a few hundred iterations. This made it feasible to draw several hundred thousand posterior samples within a few minutes on a standard multi-core CPU.

The log-likelihood function was defined in terms of patient-level imaging observations, and sampling was performed over a 14-dimensional parameter space. We initialized 500 MCMC chains with values uniformly sampled from the unit interval and ran each chain for 9000 steps. After discarding the first 6000 steps as burn-in, we flattened the remaining chains to produce a posterior sample set.

We assume that imaging observations reflect the ground truth of nodal involvement, effectively treating observed variables as perfect indicators of the underlying microscopic states. This corresponds to setting the true-positive rate \(\theta_\ell^{(\mathrm{TP})} = 1\) and the false-positive rate \(\theta_\ell^{(\mathrm{FP})} = 0\) for all LNLs. Under this assumption, the observation model simplifies to a deterministic mapping \(z_\ell^s = x_\ell^s\), which eliminates uncertainty from the diagnostic process and facilitates parameter estimation.

To explore the posterior efficiently, we combined multiple proposal strategies using differential evolution and snooker updates. These moves allowed us to sample from a correlated and constrained parameter space. Convergence was monitored using trace inspection and autocorrelation diagnostics.

==> Old_Files/Bilateral_Extension_of_BN.tex <==
\section{Bayesian Network for Bilateral Lymph Nodal Involvement}

We propose a probabilistic graphical model to represent bilateral lymphatic tumor progression in HNC. This model extends previous Bayesian networks (BNs) that were restricted to the ipsilateral neck by incorporating contralateral LNLs, while preserving anatomical interpretability and probabilistic tractability. Our formulation is influenced by recent data-driven models, such as that of \citet{ludwig_hidden_2025}, which estimate lymphatic spread using structured dependencies informed by clinical factors.

\subsection{Parameter Formulation}

Let $\mathcal{L} = \{\mathrm{I}, \mathrm{II}, \mathrm{III}, \mathrm{IV}\}$ denote the set of lymph node levels. For each level $\ell \in \mathcal{L}$ and side $s \in \{i, c\}$ (ipsilateral, contralateral), we define binary latent variables:

\begin{itemize}
    \item \( x_\ell^s \in \{0, 1\} \): A latent variable indicating the presence (1) or absence (0) of microscopic involvement in LNL \( \ell \) on side \( s \),
    \item \( z_\ell^s \in \{0, 1\} \): An observed variable indicating radiologically evident disease on imaging (e.g., CT, MRI, PET),
    \item \( T \in \{0, 1\} \): A binary variable defining primary tumour.
\end{itemize}

\subsection{Bilateral Extension}

In contrast to the ipsilateral model by \citet{pouymayou_bayesian_2019}, which defined these variables only for one side of the neck, we duplicate the latent and observed state definitions across both ipsilateral and contralateral chains, constructing two parallel subgraphs. Each subgraph has directed edges that encode anatomical progression between adjacent LNLs (e.g., $x_{\mathrm{II}}^i \rightarrow x_{\mathrm{III}}^i$). While the structure of each subgraph mirrors that of the original ipsilateral model, the key distinction lies in the presence of two parallel, side-specific chains. These evolve independently but are both influenced by shared upstream factors.

To support probabilistic inference over both observed and latent variables, we define the full joint distribution over the tumor site, latent microscopic states, and observed radiological findings.

$P(T, \mathbf{x}^i, \mathbf{x}^c, \mathbf{z}^i, \mathbf{z}^c) = P(T) \prod_{\ell \in \mathcal{L}} \prod_{s \in \{i, c\}} P(z_\ell^s \mid x_\ell^s) \cdot P(x_\ell^s \mid \text{Pa}(x_\ell^s)) $

Here, each observation $z_\ell^s$ is modeled as conditionally dependent on its corresponding latent state $x_\ell^s$ through $P(z_\ell^s \mid x_\ell^s)$, while $\text{Pa}(x_\ell^s)$ are the parents of node $x_\ell^s$ on side $s \in \{i, c\}$ for a LNL $\ell$ in the set of all levels $\mathcal{L}$.  

\subsubsection{Observational Contribution to Nodal Involvement}
% Here we should describe the P(z|x)
The association between diagnosis and microscopic spread of tumour refers to the relationship between observed states (as determined by diagnostic imaging or physical examination) and unobserved states (representing the true underlying condition). In this context, the observed state offers an observable indication of potential metastasis in a LNL. However, the unobserved state reflects the true pathological state that may not be detectable through standard diagnostic imaging. In essence, the observed state serves as a proxy for the unobserved state, but it may not always accurately reflect the pathological reality due to limitations in sensitivity and specificity of the diagnostic tools.

To formalize this relationship, let $(z_{\ell}^s , x_{\ell}^s ) \in \left\{ 0,1 \right\}$ describe the observed and unobserved states of the $i^{th}$  LNL, respectively. A healthy lymph node level is represented by a value of 0, while a malignant lymph node level is indicated by a value of 1. The conditional probability between the observed and unobserved states can be described as follows:

\begin{equation}
    P(z_{\ell}^s \mid x_{\ell}^s )= \alpha^{(1-z_{\ell}^s)(1-x_{\ell}^s )} \cdot (1-\alpha)^{z_{\ell}^s(1-x_{\ell}^s )} \cdot \beta^{z_{\ell}^s x_{\ell}^s } \cdot (1-\beta)^{(1-z_{\ell}^s)x_{\ell}^s }
\end{equation}

Where the $\alpha$ and $\beta$ parameters refer to the specificity and sensitivity of the diagnostic image modalities, respectively. For instance, if we from the diagnostic imaging observe malignant lymph nodes in the $i^{th}$ lymph node level ($P(z_{\ell}^s=1)$), but the lymph nodes is actually not malignant ($P(x_{\ell}^s=0)$), then the equation simplifies to $P(z_{\ell}^s=1 \mid x_{\ell}^s=0) = 1-\alpha$. 

\subsubsection{Parental Contributions to Nodal Involvement}

The parent set $\text{Pa}(x_\ell^s)$ for a LNL $x_\ell^s$ includes the primary tumor $T$ and any anatomically adjacent upstream LNLs, denoted $x_{\text{up}(\ell)}^s$. The conditional probability $P(x_\ell^s \mid \text{Pa}(x_\ell^s))$ models the metastatic spread and is defined differently depending on the state of the parent nodes.

The probability of microscopic involvement in level $\ell$ on side $s$, given its parents, is modeled using a "noisy-or" assumption. This assumes that each parent provides an independent chance of causing involvement. The probability that level $\ell$ remains uninvolved ($x_\ell^s=0$) is the product of probabilities that each parent fails to spread to it:

$$P(x_\ell^s=0 \mid \text{Pa}(x_\ell^s)) = (1 - b_{\ell, T}^s)^{I(T)} \prod_{k \in \text{up}(\ell)} (1 - t_{\ell, k}^s)^{I(x_k^s)}$$

where, $I(\cdot)$ is an indicator function that is 1 if its argument is true (e.g., tumor at a specific site or involvement in an upstream node) and 0 otherwise, $b_{\ell, T}^s$ (also know as the base probability) is the probability of direct spread from the primary tumor site $T$ to level $\ell$ on side $s$, and $t_{\ell, k}^s$ (also known as the transition probability) is the probability of spread from an involved upstream LNL $k$ to the downstream level $\ell$ on the same side $s$. Consequently, the probability of involvement ($x_\ell^s=1$) is simply:

$$P(x_\ell^s=1 \mid \text{Pa}(x_\ell^s)) = 1 - P(x_\ell^s=0 \mid \text{Pa}(x_\ell^s))$$

% Here we need further description of the conditional probabilities (Bayes theorem etc). --> Maybe also give some examples here with bilateral 




%¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤¤

We model lymphatic spread using a BN that encodes the probabilistic dependencies between undetected nodal involvement in multiple LNLs on both the ipsilateral ($s = i$) and contralateral ($s = c$) sides of the neck. For each LNL $\ell \in \mathcal{L} = \{\mathrm{I}, \mathrm{II}, \mathrm{III}, \mathrm{IV}\}$ and each side $s \in \{i, c\}$, the binary unobserved variable $x_\ell^s \in \{0, 1\}$ indicates whether there are tumor cells present ($1$) or not ($0$) in LNL $\ell$ on side $s$. These might be microscopic or occult tumor cell deposits that are not detectable on standard imaging modalities. In contrast, the observed variable $z_\ell^s \in \{0, 1\}$ captures the presence ($1$) or absence ($0$) of radiologically detected disease (e.g., on CT, MRI, or PET) in LNL $\ell$ on side $s$. Note that this approach allows using imperfect sensitivities and specificities, effectively accounting for false positives and false negatives.

==> Old_Files/From_Probabilities_To_Guidelines.tex <==
\section{From Probabilities to Guidelines}

While the marginal risks calculated for each LNL in section \ref{sec:risk_overview} offer valuable insights into the likelihood of occult involvement on a per-level basis, they are fundamentally limited for clinical decision-making. In clinical reality, the unobserved pattern of occult metastasis is potentially correlated among anatomically related LNLs. Therefore, a selection strategy based solely on marginal risk thresholds for individual LNLs may yield a misleading assessment of the true risk, as it does not reflect the probability that at least one excluded level harbors undetected disease.

In this section, we introduce a joint risk minimization algorithm for CTV-N definition. This approach constructs the CTV-N by iteratively adding LNLs in order of descending risk, recalculating at each step the combined probability of undetected disease across all spared (excluded) levels. In doing so, the algorithm guarantees that the total residual risk of missing disease, no matter how the microscopic pattern is distributed, remains below a user-defined risk threshold.

For each patient, we first generate a set of thinned posterior samples $\{\boldsymbol{\theta}_k\}_{k=1}^{N_s}$ from the fitted Bayesian network (e.g., by extracting every $n$th sample from the MCMC chain), representing plausible values for all model parameters. For each parameter sample $\boldsymbol{\theta}_k$, and for the patient's observed imaging findings $(\mathbf{z}^i, \mathbf{z}^c)$, we compute the full joint posterior distribution over microscopic involvement states,$P(\mathbf{x}^i, \mathbf{x}^c \mid \mathbf{z}^i, \mathbf{z}^c; \boldsymbol{\theta}_k)$ (as defined in equation \ref{eq:computing_risk}). The marginal risk of involvement for each LNL $\ell$ on side $s \in \{\text{ipsi}, \text{contra}\}$ is obtained by summing the joint posterior over all latent states where $x^s_\ell = 1$:

\begin{equation}
    \mathcal{R}^{(k)}_{\ell,s} = \sum_{\mathbf{x}^i,\, \mathbf{x}^c\, :\, x^s_\ell = 1} P(\mathbf{x}^i, \mathbf{x}^c \mid \mathbf{z}^i, \mathbf{z}^c; \boldsymbol{\theta}_k)
\end{equation}

For each lymph node level (LNL) and side, the risk assessment yields a sampled posterior risk $\mathcal{R}^{(k)}_{\ell,s}$ for every posterior parameter set $\boldsymbol{\theta}_k$. To robustly summarize the probability of microscopic involvement, we aggregate these values across all $N_s$ MCMC samples. The posterior mean risk for LNL $\ell$ and side $s$ is given by:

\begin{equation}
    \bar{\mathcal{R}}_{\ell,s} = \frac{1}{N_s} \sum_{k=1}^{N_s} \mathcal{R}^{(k)}_{\ell,s}
\end{equation}

To account for parameter uncertainty propagated from the posterior distribution, we summarize the range of plausible risks for each LNL by computing the 95\% credibility interval. This interval is defined by the empirical 2.5\textsuperscript{th} and 97.5\textsuperscript{th} percentiles of the sampled risk distribution across all posterior parameter samples:

\begin{equation}
    \mathrm{CI}_{\ell,s} = \left[\mathcal{R}^{(k_\mathrm{low})}_{\ell,s},\, \mathcal{R}^{(k_\mathrm{high})}_{\ell,s}\right]
\end{equation}

where $k_\mathrm{low}$ and $k_\mathrm{high}$ denote the percentiles corresponding to the lower and upper bounds of the desired credibility interval. We then rank all LNLs by their average risk $\bar{\mathcal{R}}_{\ell,s}$, yielding a descending-ordered list of levels most likely to harbor microscopic disease.

Starting with a hypothetical plan in which no LNLs are included in the CTV-N, we incrementally add LNLs with the highest estimated risk, recalculating at each step the cumulative risk of missing occult metastases (i.e., the total probability of disease in any excluded LNL):

\begin{equation}
    \mathcal{R}_\mathrm{missed} = \sum_{\ell \in \mathrm{excluded}} \bar{\mathcal{R}}_{\ell,s}
\end{equation}

At each iteration, we also compute the corresponding credibility interval for the missed risk, defined by the empirical bounds of the sampled posterior risk distribution for the excluded LNLs. The iterative process continues until the cumulative risk for all spared LNLs falls below a pre-specified risk threshold $\tau$:

\begin{equation}
    \mathcal{R}_\mathrm{missed} < \tau
\end{equation}

For a conservative decision criterion, we require that the \emph{upper bound} of the credibility interval for the missed risk also falls below the threshold (i.e., $\mathrm{CI}_\mathrm{missed,\, upper} < \tau$), thereby ensuring that, with high probability, the actual risk of missing microscopic disease remains within acceptable limits even in the presence of parameter uncertainty. If this condition is not satisfied, additional LNLs are included iteratively, always recalculating both the mean and credibility interval of the missed risk—until the constraint is met.

\subsection{Application on Cases of Oropharyngeal Cancer}

In this section, we present representative clinical cases of oropharyngeal cancer to illustrate how the model-based CTV-N definition compares to the conventional, guideline-based approach. Given the combinatorial complexity (there are $2^{8}$ possible treatment scenarios) we focus on the most clinically relevant and frequently encountered patterns of nodal presentation in oropharyngeal cancer patients. Table \ref{} and table \ref{} include extended listings of treatment protocols generated for different nodal involvement constellations.

In all examples, the model-based CTV-N is determined using a risk threshold of 5\%, such that the total estimated probability of occult disease in any spared nodal level does not exceed this value. Throughout, we model diagnostic performance according to the sensitivity and specificity of PET/CT combined with MRI, as previously detailed in this work.

\subsubsection{Patient 1: N0, Early-stage}

Figure \ref{fig:Treatment_Protocol_N0} compares the standard, guideline-defined CTV-N with the model-based CTV-N for a representative N0, early-stage patient. According to current clinical guidelines, elective irradiation would routinely include LNLs II and III bilaterally. In contrast, based on the  cumulative probability of missing any nodal involvement, our model suggest that we are able to omit contralateral LNL III, resulting in a total residual risk of 2.9\% for all excluded LNLs.

\subsubsection{Patient 2: N+ Ipsilateral LNL II, Early-stage}

For a patient presenting with observed nodal involvement in ipsilateral LNL II, elective irradiation according to current clinical guidelines would typically necessitate the inclusion of LNLs II–IV bilaterally. In contrast, the model-based approach indicates that ipsilateral LNL IV and contralateral LNLs II and IV may be omitted. This risk-adapted reduction in CTV-N results in an overall residual probability of undetected nodal involvement of only 3.5\% across all excluded lymph node levels. A comparative visualization of the proposed model-based CTV-N and the guideline-defined clinical CTV-N is provided in figure \ref{}.

\subsubsection{Patient 3: N+ Ipsilateral LNL II+III, Early-stage}
For a patient with confirmed nodal involvement confined to ipsilateral LNLs II and III in an early-stage scenario, the clinical guidelines generally recommend elective irradiation covering lymph node levels II–IV bilaterally. However, the model-based strategy allows elective irradiation to be restricted to ipsilateral LNLs II–IV and contralateral LNL II, with an estimated residual probability of undetected disease across all omitted nodal levels under this selective protocol of 2.1\%. A visual comparison between the model-based and clinical CTV-N definitions for this patient is illustrated in Figure \ref{}. 

\subsubsection{Patient 4: N+ Ipsilateral LNL II + Contralateral LNL II, Advanced-stage}

For an advanced-stage patient with nodal involvement observed in both ipsilateral and contralateral LNL II, clinical guidelines recommend bilateral elective irradiation of LNLs II–IV. In contrast, the model-based protocol both reduces the contralateral extent, allowing omission of LNL IV and limiting coverage to LNLs II and III, and expands the ipsilateral part of the CTV-N beyond standard practice to include LNL I, which is not routinely included under current guidelines.

These adjustments are driven by the model’s individualized risk assessment, which, for this particular case, identifies a clinically meaningful probability of nodal involvement in ipsilateral LNL I. Overall, the resulting residual risk associated with excluding the remaining nodal levels amounts to only 1.9\%. A side-by-side comparison of the model-based and guideline-defined CTV-N is shown in figure \ref{}.

\subsection{Mapping the Clinical Effect of Risk Thresholds in CTV-N Definition}

No single risk threshold can claim to be “correct” for all patients or all institutions. Instead, it reflects a nuanced compromise between safety and quality of life. The choice of threshold may depend on institutional philosophy, patient preferences, and evolving evidence regarding acceptable levels of residual risk. A sensitivity analysis provides transparency regarding how different risk tolerance levels translate into changes in the extent of irradiation and the corresponding residual risk of nodal involvement. This section provides a side-by-side comparison of CTV-N definitions across multiple risk thresholds, using the same patient examples introduced earlier to highlight the resulting changes in treatment recommendations.

\subsubsection{Patient 1: N0, Early-stage}

For this representative early-stage (N0) patient, we explored how varying the risk threshold for occult nodal disease influences the extent of elective nodal irradiation. Using a moderate risk threshold of 5\%, the model-based protocol recommends elective irradiation of ipsilateral LNLs I–IV and contralateral LNL II, resulting in a residual risk of 2.9\% for harboring disease in any of the excluded nodal levels.

Adjusting the threshold upward to 10\% allows for further de-escalation, enabling complete omission of the contralateral neck from the CTV-N. This substantially reduces the irradiated volume, with only a modest increase in total residual risk to 6.8\%. Conversely, adopting a more conservative threshold of 2\% requires broader coverage—expanding the CTV-N to include ipsilateral LNLs I–IV and maintaining contralateral LNL II—lowering the residual risk to just 0.8\% at the expense of treating additional healthy tissue. For context, if all LNLs were omitted from the CTV-N, with only the high- and intermediate-risk CTVs were irradiated, the residual risk of nodal involvement would rise dramatically to 51.6\%.

Figure \ref{} illustrates these trade-offs, plotting the residual risk associated with each risk-adapted protocol alongside the corresponding patterns of nodal coverage. The results highlight how small changes in risk tolerance can meaningfully alter both the recommended CTV-N and the balance between disease control and tissue sparing.

% The different treatment protocols for different risk threshold can be seen figure \ref{}.

\subsubsection{Patient 2: N+ Ipsilateral LNL II, Early-stage}

\subsubsection{Patient 3: N+ Ipsilateral LNL II+III, Early-stage}

\subsubsection{Patient 4: N+ Ipsilateral LNL II + Contralateral LNL II, Advanced-stage}

% ###############################################################

\section{From Probabilities to Guidelines}

While the marginal risks calculated for each LNL in section \ref{sec:risk_overview} offer valuable insights into the likelihood of occult involvement on a per-level basis, they are fundamentally limited for clinical decision-making. In clinical reality, the unobserved pattern of occult metastasis is potentially correlated among anatomically related LNLs. Therefore, a selection strategy based solely on marginal risk thresholds for individual LNLs may yield a misleading assessment of the true risk, as it does not reflect the probability that at least one excluded level harbors undetected disease.

In this section, we introduce a joint risk minimization algorithm for CTV-N definition. This approach constructs the CTV-N by iteratively adding LNLs in order of descending risk, recalculating at each step the combined probability of undetected disease across all spared (excluded) levels. In doing so, the algorithm guarantees that the total residual risk of missing disease, no matter how the microscopic pattern is distributed, remains below a user-defined risk threshold.

For each patient, we first generate a set of thinned posterior samples $\{\boldsymbol{\theta}_k\}_{k=1}^{N_s}$ from the fitted Bayesian network (e.g., by extracting every $n$th sample from the MCMC chain), representing plausible values for all model parameters. For each parameter sample $\boldsymbol{\theta}_k$, and for the patient's observed imaging findings $(\mathbf{z}^i, \mathbf{z}^c)$, we compute the full joint posterior distribution over microscopic involvement states,$P(\mathbf{x}^i, \mathbf{x}^c \mid \mathbf{z}^i, \mathbf{z}^c; \boldsymbol{\theta}_k)$ (as defined in equation \ref{eq:computing_risk}). The marginal risk of involvement for each LNL $\ell$ on side $s \in \{\text{ipsi}, \text{contra}\}$ is obtained by summing the joint posterior over all latent states where $x^s_\ell = 1$:

\begin{equation}
    \mathcal{R}^{(k)}_{\ell,s} = \sum_{\mathbf{x}^i,\, \mathbf{x}^c\, :\, x^s_\ell = 1} P(\mathbf{x}^i, \mathbf{x}^c \mid \mathbf{z}^i, \mathbf{z}^c; \boldsymbol{\theta}_k)
\end{equation}

For each lymph node level (LNL) and side, the risk assessment yields a sampled posterior risk $\mathcal{R}^{(k)}_{\ell,s}$ for every posterior parameter set $\boldsymbol{\theta}_k$. To robustly summarize the probability of microscopic involvement, we aggregate these values across all $N_s$ MCMC samples. The posterior mean risk for LNL $\ell$ and side $s$ is given by:

\begin{equation}
    \bar{\mathcal{R}}_{\ell,s} = \frac{1}{N_s} \sum_{k=1}^{N_s} \mathcal{R}^{(k)}_{\ell,s}
\end{equation}

To account for parameter uncertainty propagated from the posterior distribution, we summarize the range of plausible risks for each LNL by computing the 95\% credibility interval. This interval is defined by the empirical 2.5\textsuperscript{th} and 97.5\textsuperscript{th} percentiles of the sampled risk distribution across all posterior parameter samples:

\begin{equation}
    \mathrm{CI}_{\ell,s} = \left[\mathcal{R}^{(k_\mathrm{low})}_{\ell,s},\, \mathcal{R}^{(k_\mathrm{high})}_{\ell,s}\right]
\end{equation}

where $k_\mathrm{low}$ and $k_\mathrm{high}$ denote the percentiles corresponding to the lower and upper bounds of the desired credibility interval. We then rank all LNLs by their average risk $\bar{\mathcal{R}}_{\ell,s}$, yielding a descending-ordered list of levels most likely to harbor microscopic disease.

Starting with a hypothetical plan in which no LNLs are included in the CTV-N, we incrementally add LNLs with the highest estimated risk, recalculating at each step the cumulative risk of missing occult metastases (i.e., the total probability of disease in any excluded LNL):

\begin{equation}
    \mathcal{R}_\mathrm{missed} = \sum_{\ell \in \mathrm{excluded}} \bar{\mathcal{R}}_{\ell,s}
\end{equation}

At each iteration, we also compute the corresponding credibility interval for the missed risk, defined by the empirical bounds of the sampled posterior risk distribution for the excluded LNLs. The iterative process continues until the cumulative risk for all spared LNLs falls below a pre-specified risk threshold $\tau$:

\begin{equation}
    \mathcal{R}_\mathrm{missed} < \tau
\end{equation}

For a conservative decision criterion, we require that the \emph{upper bound} of the credibility interval for the missed risk also falls below the threshold (i.e., $\mathrm{CI}_\mathrm{missed,\, upper} < \tau$), thereby ensuring that, with high probability, the actual risk of missing microscopic disease remains within acceptable limits even in the presence of parameter uncertainty. If this condition is not satisfied, additional LNLs are included iteratively, always recalculating both the mean and credibility interval of the missed risk, until the constraint is met.

==> Old_Files/Mathematics_Of_BN.tex <==
Building on Pouymayou et al. [15], this study proposes a similar approach. In this study we categories the bayesian network into three elements. 

\begin{enumerate}
    \item Correlation between diagnosis and sub-clincal disease
    \item Metastasis from primary tumour to lymph node levels
    \item Metastasis between lymph node levels
\end{enumerate}

Firstly , the association between diagnosis and sub-clinical disease refers to the relationship between observed states (as determined by diagnostic imaging or physical examination) and unobserved states (representing the true underlying condition). In this context, the observed state offers an observable indication of potential metastasis in a lymph node level. However, the unobserved state reflects the true pathological state that may not be detectable through standard diagnostic imaging. In essence, the observed state serves as a proxy for the unobserved state, but it may not always accurately reflect the pathological reality due to limitations in sensitivity and specificity of the diagnostic tools.

To formalize this relationship, let $(\Delta_{i},\Theta_{i}) \in \left\{ 0,1 \right\}$ describe the observed and unobserved states of the $i^{th}$  LNL, respectively. A healthy lymph node level is represented by a value of 0, while a malignant lymph node level is indicated by a value of 1. The conditional probability between the observed and unobserved states can be described as follows:

\begin{equation}
    \mathbb{P}(\Theta_{i}=\theta |\Delta_{i}=\delta) = \alpha^{(1-\theta)(1-\delta)} \cdot (1-\alpha)^{\theta(1-\delta)} \cdot \beta^{\theta\delta} \cdot (1-\beta)^{(1-\theta)\delta}
\end{equation}

Where the $\alpha$ and $\beta$ parameters refer to the specificity and sensitivity of the diagnostic image modalities, respectively. For instance, if we from the diagnostic imaging observe malignant lymph nodes in the $i^{th}$ lymph node level ($\mathbb{P}(\Theta_{i}=1)$), but the lymph nodes is actually not malignant ($\mathbb{P}(\Delta_{i}=0)$), then the equation simplifies to $\mathbb{P}(\Theta_{i}=1 | \Delta_{i}=0) = 1-\alpha$. 

Secondly , the primary tumour ($\Psi$), and its influence on lymph node level involvement is represented by the directed arcs connecting it to the $i^{th}$ LNL ($\Delta_{i}$), as illustrated in figure 2. The probabilistic dependencies of the direct metastatic spread from the primary tumour to the lymph node levels is denoted by the spread probability $\mathbb{P}_{\Psi_{i}}$. The spread probability $\mathbb{P}_{\Psi_{i}}$ is described through the conditional probability:

\begin{equation}
    \mathbb{P}(\Delta_{i}=\delta| \Psi=\psi) = (\mathbb{P}_{\Psi_{i}})^{\delta\psi} \cdot (1-\mathbb{P}_{\Psi_{i}})^{\psi(1-\delta)} \cdot (1-\psi)^{1-\delta} 
\end{equation}

Where, $\Psi \in {0,1}$ and $\delta_{i} \in {0,1}$. If we, for instance, observe no microscopic involvement of the lymph node level ($\mathbb{P}(\delta_{i}=0)$), then the equation simplifies to $\mathbb{P}(\delta_{i}=0 | \Psi=1) = 1-\mathbb{P}_{\Psi_{i}}$

Thirdly, the inter-nodal spread is influenced by lymphatic drainage patterns, where, for example, lymph node level III receives efferent lymphatic drainage from lymph node level II. These relationships can be represented by directed arcs connecting the nodes sequentially within a network, as shown in figure 3. However, it becomes evident that the parameter space in bayesian networks can quickly become high-dimensional; for instance, with just four nodes, there would be $2^{4}$ potential parameter combinations. This exponential growth significantly increases the complexity and computational requirements of the model. Therefore, to address the challenge of parameter explosion  in bayesian networks, particularly when modelling complex causal relationships, we propose the use of Noisy-OR gates as a strategy to reduce the dimensionality of the parameter space. The Noisy-OR is given by:

\begin{equation}
    \mathbb{P}(\Delta_{i}^{1}|\Upsilon) = 1-\prod_{i:\Upsilon_{i} \in \Upsilon} (1-\upsilon_{i})
\end{equation}

Where $\Upsilon$ denotes the subset of parent nodes that influence the respective child node $\Delta_{i}$, $\Upsilon_{i}$ denotes an individual parent node within the subset $\Upsilon$, $\upsilon_{i}$ is the probability that the parent node $\Upsilon_{i}$ will cause $\Delta_{i}$ to be in the same state (either 0 or 1) as $\Upsilon_{i}$, and $\prod_{i:\Upsilon_{i} \in \Upsilon} (1-\upsilon_{i})$ captures the joint probability that none of the parent nodes $\Upsilon_{i}$ contribute to $\Delta_{i}$ being in state 1, and subtracting this product from 1 gives the probability that at least one parent node causes $\Delta_{i}$ to be in state 1. It is worth noting that for $\Delta_{i}^{0}$

 the Noisy-OR simplifies to $\mathbb{P}(\Delta_{i}^{0}|\Upsilon) = \prod_{i:\Upsilon_{i} \in \Upsilon} (1-\upsilon_{i})$. Let us for instance say, that we are interested in knowing the probability of observing nodal involvement of lymph node level III ($\mathbb{P}(\Delta_{III}=1)$), given no involvement of lymph node level II ($\mathbb{P}(\Delta_{II}=0 )$), we describe the Noisy-OR as ($\mathbb{P}(\Delta_{II}=0)|\Delta_{II}=0, \Psi=1) = \mathbb{P}(\Psi_{III})$), meaning it only depends on the spread probability from primary tumour to lymph node level III. The full parameterised conditional probability table becomes:

 
\[
 \mathbb{P}(\Delta_{i}^{1}|\Upsilon) = 
  \begin{cases} 
   1-(1-\mathbb{P}_{\Delta_{ij}})(1-\mathbb{P}_{\Psi_{i}}), & \textit{if } \Delta_{i} = 1, \Psi = 1 \\
   \mathbb{P}_{\Psi_{i}},     & \textit{if } \Delta_{i} = 0, \Psi = 1
   \\
   \mathbb{P}_{\Delta_{ij}},  & \textit{if } \Delta_{i} = 1, \Psi = 0
   \\
   0,    & \textit{if } \Delta_{i} = 0, \Psi = 0
  \end{cases}
\]

==> Old_Files/Old_Bilateral_Section.tex <==
\subsection{Bilateral Extension}

In contrast to the ipsilateral model by \citet{pouymayou_bayesian_2019}, which defined these variables only for one side of the neck, we duplicate the latent and observed state definitions across both ipsilateral and contralateral chains, constructing two parallel subgraphs. Each subgraph has directed edges that encode anatomical progression between adjacent LNLs (e.g., $x_{\mathrm{II}}^i \rightarrow x_{\mathrm{III}}^i$). While the structure of each subgraph mirrors that of the original ipsilateral model, the key distinction lies in the presence of two parallel, side-specific chains. These evolve independently but are both influenced by shared upstream factors.

% We need so go directly into the joint probability, and then afterward describe what Pa(x) is. 

To support probabilistic inference over both observed and latent variables, we define the full joint distribution over the tumor site, latent microscopic states, and observed radiological findings.

\begin{equation}
P(T, \mathbf{x}^i, \mathbf{x}^c, \mathbf{z}^i, \mathbf{z}^c) = P(T) \prod_{\ell \in \mathcal{L}} \prod_{s \in {i, c}} P(x_\ell^s \mid \text{Pa}(x_\ell^s)) \cdot P(z_\ell^s \mid x_\ell^s)
\end{equation}

Here, $\text{Pa}(x_\ell^s) \subseteq \{T, x_{\text{upstream}}^s\}$ are the parents of each node on side $s$. This decomposition generalizes the factorization in the ipsilateral model by allowing both sides to be modeled symmetrically but separately. This factorization explicitly excludes any term such as $P(x_\ell^c \mid x_\ell^i)$; the two sides evolve independently except through shared upstream influences like tumor origin. 

% Describe here, in relation to the factorization, the term Pa(x)
Since $\text{Pa}(x_\ell^s)$ describes the parent nodes ... %we need to write here the definition of the Pa(x) 

% describe P(x|T) --> The spread from primary tumour to each LNL --> We also need to describe the conditional probability --> We are interested in the probability of microscopic involvement based on the examination of the macroscopic state and the primary tumor

% Describe P(x|x,T) --> The spread between LNLs --> we are interested in how this probability depends on, i.e. whether or not level II harbors macroscopic metastases.

==> Old_Files/Overview_Of_Computed_Risks.tex <==
\subsection{Overview of Risk Estimates for Nodal Involvement} \label{sec:risk_overview}

For patients with a radiologically negative (N0) neck, the predicted probability of harbouring microscopic tumour involvement varies substantially across LNLs and tumour stage. On the ipsilateral side, early-stage tumours are associated with a risk of 1.1\% in LNL I, which rises sharply to 47.8\% in LNL II, then decreases to 8.2\% in LNL III and falls below 1\% in LNL IV. In advanced-stage tumours, these probabilities increase further to 4.0\% in LNL I, 57.6\% in LNL II, 12.6\% in LNL III, and 1.8\% in LNL IV.

On the contralateral side, the risks are generally (considerably) lower, but a clear dependence on both tumour stage and LNL remains evident. For early-stage tumours, the probabilities are below 1\% in LNL I, 4.4\% in LNL II, below 1\% in LNL III, and below 1\% in LNL IV. In advanced-stage tumours, the risk increases substantially in LNL II to 18.1\% and in LNL III to 2.4\%, while LNL I and IV remain below 1\%.

Once nodal involvement is observed on imaging, the risk of nodal involvement changes markedly, with increased probabilities observed for adjacent and downstream LNLs. For example, when ipsilateral LNL II is found to be involved, the probability of downstream involvement in ipsilateral LNL III nearly doubles, rising from 8.2\% to 14.4\% in early-stage tumours and from 12.6\% to 19.7\% in advanced-stage tumours. A similar pattern is observed contralaterally, if contralateral LNL II is positive on imaging, the risk of microscopic disease in contralateral LNL III increases from less than 0.1\% to 3.6\% in early-stage tumours and from 2.4\% to 7.0\% in advanced-stage tumours.

For a complete overview of the computed risk of nodal involvement across all clinically relevant patterns of observed nodal involvements on diagnostic imaging, we refer the readers to table \ref{tab:Results}.

==> Old_Files/Risk_Assessment.tex <==
\subsection{Risk Assessment}

We compute the risk of nodal involvement for any pattern or specific LNL, conditional on an individual patient’s observed diagnosis. For a patient with observed imaging findings $\mathbf{z}^i, \mathbf{z}^c$, the posterior probability of any pair of latent nodal involvement states $(\mathbf{x}^i, \mathbf{x}^c)$ is given by Bayes’ theorem:

\begin{equation} \label{eq:computing_risk}
P(\mathbf{x}^i, \mathbf{x}^c \mid \mathbf{z}^i, \mathbf{z}^c, T; \boldsymbol{\theta}) =
\frac{
    P(\mathbf{x}^i, \mathbf{x}^c \mid T; \boldsymbol{\theta})\,
    P(\mathbf{z}^i \mid \mathbf{x}^i)\,
    P(\mathbf{z}^c \mid \mathbf{x}^c)
}{
    \displaystyle\sum_{\mathbf{x}^{i'} \in \mathcal{X}^i}\sum_{\mathbf{x}^{c'} \in \mathcal{X}^c}
    P(\mathbf{x}^{i'}, \mathbf{x}^{c'} \mid T; \boldsymbol{\theta})\,
    P(\mathbf{z}^i \mid \mathbf{x}^{i'})\,
    P(\mathbf{z}^c \mid \mathbf{x}^{c'})
}
\end{equation}

Here, the numerator represents the product of the joint prior probability for the given latent state and the likelihood of the observed imaging findings for that state. The denominator is a normalization constant ensuring the posterior sums to one. Here, the prime notation ($\mathbf{x}^{i'}$, $\mathbf{x}^{c'}$) in the denominator indicates summation over all possible configurations of the latent states, different from the specific $(\mathbf{x}^i, \mathbf{x}^c)$ considered in the numerator.

To compute the marginal risk for involvement of a specific lymph node level, e.g., the probability that ipsilateral LNL III is involved, we sum the posterior probability over all configurations where $x_\text{III}^i = 1$:

\begin{equation}
P(x^i_\text{III} = 1 \mid \mathbf{z}^i, \mathbf{z}^c, T; \boldsymbol{\theta}) =
\sum_{x_{III}^i = 1}
\sum_{\mathbf{x}^c \in \mathcal{X}^c}
P(\mathbf{x}^i, \mathbf{x}^c \mid \mathbf{z}^i, \mathbf{z}^c, T; \boldsymbol{\theta})
\end{equation}

This same marginalization approach applies for any single node or combination of nodes. In practice, the risk for a given pattern is obtained by enumerating all possible $(\mathbf{x}^i, \mathbf{x}^c)$, evaluating the posterior for each, and summing over those that match the involvement criteria.

Unlike during parameter estimation, where we treated the observed imaging findings as ground truth (i.e., assumed perfect sensitivity and specificity), risk assessment for individual patients instead uses the true sensitivity and specificity of the diagnostic modality. In Denmark, diagnosis of nodal involvement is most often established by PET/CT combined MRI. However, to our knowledge, there are no published studies that report the sensitivity and specificity of PET/CT combined with MRI for this purpose. Therefore, we parameterized the observation model $P(\mathbf{z}^s \mid \mathbf{x}^s)$ using a sensitivity of 0.71 and a specificity of 0.90 for PET/CT alone, as reported by \citet{guedj_fdg_2024}.


==> Old_Files/related_works.tex <==
% Several previous studies have investigated strategies to reduce elective irradiation volumes in head and neck cancer, aiming to lower treatment-related toxicity while preserving regional control. These efforts include rule-based modifications of existing contouring guidelines, probabilistic modeling to estimate individualized risk of occult nodal involvement, and ongoing clinical trials evaluating both surgical-staging–guided and model-based approaches to volume de-escalation.

% A recent study by \citet{weissmann_reduction_2021} proposed a revised elective nodal contouring strategy for definitive radiotherapy in locally advanced head and neck squamous cell carcinoma, omitting LNLs with historically low involvement rates, particularly levels I and IV, based on the primary tumor site and disease extent. The approach was informed by a large institutional dataset on patterns of spread and applied uniformly within each clinical subgroup. In a dosimetric comparison of 30 patients, the volume de-escalated treatment plans maintained target coverage while decreasing the irradiated volume of surrounding normal tissues, leading to lower calculated mean doses to several organs-at-risk. Although this approach can simplify and standardize volume reduction, it does not account for patient-specific risks and therefore may not achieve the same degree of individualized sparing as probabilistic, case-by-case strategies such as the one presented in our work. 

% An extensive literature-based review by \citet{al-mamgani_contralateral_2017} evaluated a specific form of spatial volume de-escalation—omitting contralateral elective nodal irradiation, in well, lateralized oropharyngeal carcinoma. Across 11 retrospective series (n = 1116), the mean contralateral regional failure (cRF) rate was 2.4\%, with isolated cRF in 1.7\%. Midline involvement was the strongest predictor of recurrence, with a pooled cRF of 12.1\%, markedly higher than in lateralized cases. In our sensitivity analysis of midline-crossing tumors, contralateral omission was only permissible at risk thresholds of 10\% or greater, highlighting that the extent of elective coverage is inherently linked to the maximum recurrence risk considered acceptable. Both analyses therefore indicate that, for midline extension, the decision between bilateral and unilateral treatment depends on the acceptable recurrence risk, with contralateral sparing only justifiable if that threshold is set at around 10\% or higher.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% However, the approach most closely related to ours is that of \citet{ludwig_hidden_2025}, who used a Hidden Markov Model (HMM) of bilateral lymphatic spread in oropharyngeal squamous cell carcinoma to estimate patient-specific probabilities of contralateral occult involvement. In their study, the CTV-E were defined by estimating the contralateral risk for each patient and including or omitting contralateral LNLs based on whether this probability exceeded a fixed 5\% risk threshold. Using this criterion, midline-extending tumors consistently yielded contralateral occult disease probabilities above 5\%, leading to a uniform recommendation for bilateral ENI in this subgroup.

% While our findings for midline-extending cases generally agree with theirs, in that all patients exceeded the 5\% contralateral risk threshold, the way risk is assessed and applied differs fundamentally. Ludwig and colleagues' approach considers the marginal risk of occult involvement for a single group of contralateral LNLs, without accounting for the correlated risk that arises when multiple levels, on one or both sides, are omitted simultaneously. Therefore, the results of the two studies are not directly comparable, as the underlying risk definitions and scope of target adaptation differ substantially. Nevertheless, both approaches point to the same overarching conclusion for midline-extending tumors, namely, that contralateral omission is rarely justified at low to moderate risk thresholds, while our framework expands this reasoning to guide comprehensive, patient-specific CTV-E adaptation across the entire neck.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Increasing clinical data suggest that large, bilateral nodal volumes may not be necessary in all head and neck cancer cases. With the introduction of high-resolution cross-sectional imaging, sentinel node procedures, and an improved understanding of lymphatic spread patterns, the risk of isolated regional failure in electively treated volumes, particularly in the contralateral neck of lateralized tumours, has been shown to be very low. Several strategies for volume de-escalation have therefore been investigated. Selective omission of low-risk nodal levels based on site-specific patterns of spread has been proposed in revised contouring guidelines and simulated planning studies, demonstrating substantial sparing of organs-at-risk without compromising coverage of high-risk areas \cite{weissmann_reduction_2021,garcia-anaya_dose_2023}. Elective irradiation restricted to a single neck side in well-lateralized oropharyngeal and oral cavity cancers has consistently yielded low contralateral failure rates below 5\% in retrospective series and meta-analyses \cite{al-mamgani_contralateral_2017,garcia-anaya_dose_2023}. More recently, functional imaging and surgical staging approaches, such as SPECT/CT-guided lymphatic mapping or sentinel node biopsy, have enabled tailoring of CTV-E to individual drainage patterns, with prospective trials reporting contralateral failure rates of 0-3\% and significant reductions in xerostomia, dysphagia, and long-term feeding-tube dependence \cite{veij_mapping_2019,veij_spectct-guided_2020,de_veij_spectct-guided_2018}.

% While these studies are based on different methods, ranging from rule-based level omission, to functional lymphatic imaging, to surgical staging, the underlying premise is the same: volume de-escalation can reduce treatment-related toxicity while maintaining low rates of regional failure, provided that patient selection is accurate. Our work builds directly on this principle, but addresses a key limitation of prior approaches by replacing fixed, population-based assumptions with a probabilistic model that quantifies the risk of occult involvement in each LNL for the individual patient. This allows diagnostic information and tumour characteristics, to be combined into a continuous, interpretable risk estimate that can be directly inspected and validated by clinicians, which is advantageous in a setting where transparency is essential for clinical adoption.

==> Placeholder.tex <==
We model lymphatic tumor progression using a structured Bayesian network (BN) that encodes the probabilistic dependencies between microscopic tumor involvement in multiple lymph node levels (LNLs) on both the ipsilateral ($s = i$) and contralateral ($s = c$) sides of the neck. For each LNL $\ell \in \mathcal{L} = \{\mathrm{I}, \mathrm{II}, \mathrm{III}, \mathrm{IV}\}$ and each side $s \in \{i, c\}$, the binary latent variable $x_\ell^s \in \{0, 1\}$ indicates whether there is microscopic tumor cell presence ($1$) or not ($0$) in LNL $\ell$ on side $s$. The observed variable $z_\ell^s \in \{0, 1\}$ captures the presence ($1$) or absence ($0$) of radiologically apparent disease (e.g., on CT, MRI, or PET) in LNL $\ell$ on side $s$. The tumor site or T-category is represented by the variable $T$.

The Bayesian network is structured such that each $x_\ell^s$ node is connected to its anatomical parent(s), most commonly the preceding nodal level on the same side ($x_{\ell-1}^s$ for $\ell > 1$) and the primary tumor variable $T$. This structure reflects the anatomical progression pathways for tumor spread through the lymphatic system and allows for explicit modeling of dependencies between neighboring LNLs as well as the influence of the primary tumor.

For notational clarity, we define the vectors $\mathbf{x}^s = (x^s_\ell)_{\ell \in \mathcal{L}}$ and $\mathbf{z}^s = (z^s_\ell)_{\ell \in \mathcal{L}}$ to represent the full latent and observed state across all LNLs on side $s$, respectively. The joint prior distribution over all microscopic involvement states on both sides is given by

\begin{equation}
P(\mathbf{x}^i, \mathbf{x}^c) = \sum_{T} P(T) \, P(\mathbf{x}^i \mid T) \, P(\mathbf{x}^c \mid T)
\label{eq:bn_joint_prior}
\end{equation}

where $P(T)$ is the prior probability of the tumor site, and the conditional probability of a full involvement pattern on side $s$ given $T$ is factorized according to the BN structure:

\begin{equation}
P(\mathbf{x}^s \mid T) = \prod_{\ell \in \mathcal{L}} P(x^s_\ell \mid \mathrm{Pa}(x^s_\ell), T)
\end{equation}

Here, $\mathrm{Pa}(x^s_\ell)$ denotes the parent nodes of $x^s_\ell$, typically including $x^s_{\ell-1}$ for $\ell > 1$ and the tumor variable $T$.



We model the radiological findings such that, under the assumption of conditional independence, the probability of a radiological finding in any LNL depends only on its true microscopic involvement and is unaffected by the state of other levels:

\begin{equation}
P(\mathbf{z}^s \mid \mathbf{x}^s) = \prod_{\ell \in \mathcal{L}} P(z^s_\ell \mid x^s_\ell)
\end{equation}

where $P(z^s_\ell \mid x^s_\ell)$ specifies the probability of a positive or negative radiological result in lymph node level $\ell$ conditional on its true microscopic involvement, reflecting the sensitivity and specificity of the diagnostic imaging modality. Given observed imaging findings $\mathbf{z}^i$ and $\mathbf{z}^c$, we compute the posterior distribution over all latent microscopic involvement configurations using Bayes' theorem:

\begin{equation}
P(\mathbf{x}^i, \mathbf{x}^c \mid \mathbf{z}^i, \mathbf{z}^c) = 
\frac{P(\mathbf{x}^i, \mathbf{x}^c) \, P(\mathbf{z}^i \mid \mathbf{x}^i) \, P(\mathbf{z}^c \mid \mathbf{x}^c)}{\sum_{\mathbf{x}^i,\, \mathbf{x}^c} P(\mathbf{x}^i, \mathbf{x}^c) \, P(\mathbf{z}^i \mid \mathbf{x}^i) \, P(\mathbf{z}^c \mid \mathbf{x}^c)}
\end{equation}

where the denominator ensures normalization across all possible combinations of microscopic involvement on both sides. This formulation enables the explicit computation of marginal and conditional probabilities for any subset of LNLs or clinically relevant pattern.


==> figures.tex <==

%Graphical representation of the Bilateral Bayesian Network
\begin{figure}[H]
\centering
\includegraphics[width=0.8\textwidth]{figures/BN_Graph.png}
\caption{Structure of the Bilateral Bayesian Network modeling lymphatic drainage. The unobserved variables $x^s_k$ represent the true involvement status of the $\mathrm{k}^{th}$ LNL on side $s \in {i,c}$, while $z^s_k$ denotes the observed status as defined by diagnostic imaging. $T$ represents the primary tumour. Each directed arc encodes either a base probability ($b^s_k$) or a transition probability ($t^s_k$).}
\label{BN_Graph}
\end{figure}

% Upset plots for visualisation of the spread patterns
\begin{figure}[H]
    \centering
    \begin{subfigure}{0.9\textwidth} % Reduce the width slightly
        \caption{}
        \label{fig:ipsilateral_upset}
        \includegraphics[width=\textwidth]{figures/upset_plot_ipsilateral.png}
    \end{subfigure}
    
    \vspace{0.3cm} % Adjust vertical space if needed

    \begin{subfigure}{0.9\textwidth} % Reduce the width slightly
        \caption{}
        \label{fig:contralateral_upset}
        \includegraphics[width=\textwidth]{figures/upset_plot_contralateral.png}
    \end{subfigure}        

    \caption{Upset plots illustrating the patterns of nodal involvement. (\textbf{a}) UpSet plot of lymphatic nodal spread patterns for different involvement patterns in early- and advanced-stage ipsilateral LNLs. (\textbf{b}) UpSet plot of lymphatic nodal spread patterns for different involvement patterns in early- and advanced-stage contralateral LNLs. The left panels in each figure showcase the prevalence of involvement for each LNL individually, while the main panels highlight the most frequent patterns of simultaneous nodal involvement. }
    \label{fig:UpSet_plot_data_characteristics}
\end{figure}

% TREATMENT GUIDELINES FOR N0

\begin{figure}[H]
\centering
\scriptsize

\begin{subfigure}{0.48\linewidth}
    \centering
    \caption{Current Clinical Practice (DAHANCA)}
    \label{fig:Treatment_Protocols_N0_Clinical}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_Clinical_Protocol.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Clinical_Protocol.png}
    \end{minipage}
\end{subfigure}
\hfill
\begin{subfigure}{0.48\linewidth}
    \centering
    \caption{Model-based for 2\% Risk Threshold}
    \label{fig:Treatment_Protocols_N0_2}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_2_procent.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_2_procent.png}
    \end{minipage}

\end{subfigure}

\vspace{1mm}

\begin{subfigure}{0.48\linewidth}
    \centering
    \caption{Model-based for 5\% Risk Threshold}
    \label{fig:Treatment_Protocols_N0_5}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_5_procent.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_5_procent.png}
    \end{minipage}
\end{subfigure}
\hfill
\begin{subfigure}{0.48\linewidth}
    \centering
    \caption{Model-based for 8\% Risk Threshold}
    \label{fig:Treatment_Protocols_N0_8}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_8_procent.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_8_procent.png}
    \end{minipage}
    
\end{subfigure}

\vspace{1mm}

\begin{subfigure}{0.48\linewidth}
    \centering
    \caption{Model-based for 10\% Risk Threshold}
    \label{fig:Treatment_Protocols_N0_10}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_10_procent.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_10_procent.png}
    \end{minipage}
    
\end{subfigure}
\hfill
\begin{subfigure}{0.48\linewidth}
    \centering
    \caption{Model-based for 12\% Risk Threshold}
    \label{fig:Treatment_Protocols_N0_12}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_12_procent.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_12_procent.png}
    \end{minipage}
    
\end{subfigure}

\vspace{1mm}

\begin{subfigure}{0.48\linewidth}
    \centering
    \caption{Model-based for 15\% Risk Threshold}
    \label{fig:Treatment_Protocols_N0_15}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_15_procent.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_15_procent.png}
    \end{minipage}
    
\end{subfigure}
\hfill
\begin{subfigure}{0.48\linewidth}
    \centering
    \caption{Model-based for 20\% Risk Threshold}
    \label{fig:Treatment_Protocols_N0_20}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_20_procent.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_20_procent.png}
    \end{minipage}
    
\end{subfigure}

\caption{Estimated elective nodal irradiation strategies for a patient with an early-stage central oropharyngeal tumour and N0 disease under varying risk thresholds. LNLs above the inclusion threshold are shown in orange (included into the CTV-E), while LNLs below the threshold are shown in gray (excluded from treatment)}
\label{fig:Treatment_Protocols_N0}
\end{figure}


% TREATMENT GUIDELINES FOR N+ Ipsilateral LNL II

\begin{figure}[H]
\centering
\scriptsize

\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Current Clinical Practice (DAHANCA)}
    \label{fig:Treatment_Protocols_N+_II_Clinical}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_Clinical_Protocol_N+_II.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Clinical_Protocol_N+_II.png}
    \end{minipage}
    
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 2\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_2}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_2_procent_N+_II.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_2_procent_N+_II.png}
    \end{minipage}
    
\end{subfigure}

\vspace{1mm}

\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 5\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_5}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_5_procent_N+_II.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_5_procent_N+_II.png}
    \end{minipage}
    
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 8\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_8}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_8_procent_N+_II.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_8_procent_N+_II.png}
    \end{minipage}
    
\end{subfigure}

\vspace{1mm}

\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 10\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_10}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_10_procent_N+_II.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_10_procent_N+_II.png}
    \end{minipage}
    
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 12\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_12}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_12_procent_N+_II.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_12_procent_N+_II.png}
    \end{minipage}
    
\end{subfigure}

\vspace{1mm}

\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 15\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_15}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_15_procent_N+_II.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_15_procent_N+_II.png}
    \end{minipage}
    
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 20\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_20}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_20_procent_N+_II.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_20_procent_N+_II.png}
    \end{minipage}
    
\end{subfigure}

\caption{Estimated elective nodal irradiation strategies for a patient with an early-stage central oropharyngeal tumour and N+ disease in ipsilateral LNL II under varying risk thresholds. LNLs above the inclusion threshold are shown in orange (included into the CTV-E), while LNLs below the threshold are shown in gray (excluded from treatment)}
\label{fig:Treatment_Protocols_N+_II}
\end{figure}



% TREATMENT GUIDELINES FOR N+ Ipsilateral LNL II + III

\begin{figure}[H]
\centering
\scriptsize

\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Current Clinical Practice (DAHANCA)}
    \label{fig:Treatment_Protocols_N+_II_III_Clinical}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_Clinical_Protocol_N+_II_III.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Clinical_Protocol_N+_II_III.png}
    \end{minipage}
    
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 2\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_III_2}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_2_procent_N+_II_III.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_2_procent_N+_II_III.png}
    \end{minipage}
    
\end{subfigure}

\vspace{1mm}

\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 5\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_III_5}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_5_procent_N+_II_III.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_5_procent_N+_II_III.png}
    \end{minipage}
    
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 8\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_III_8}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_8_procent_N+_II_III.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_8_procent_N+_II_III.png}
    \end{minipage}
    
\end{subfigure}

\vspace{1mm}

\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 10\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_III_10}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_10_procent_N+_II_III.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_10_procent_N+_II_III.png}
    \end{minipage}
    
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 12\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_III_12}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_12_procent_N+_II_III.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_12_procent_N+_II_III.png}
    \end{minipage}
    
\end{subfigure}

\vspace{1mm}

\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 15\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_III_15}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_15_procent_N+_II_III.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_15_procent_N+_II_III.png}
    \end{minipage}
    
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 20\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_III_20}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_20_procent_N+_II_III.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_20_procent_N+_II_III.png}
    \end{minipage}
    
\end{subfigure}

\caption{Estimated elective nodal irradiation strategies for a patient with an early-stage central oropharyngeal tumour and N+ disease in ipsilateral LNL II and III under varying risk thresholds. LNLs above the inclusion threshold are shown in orange (included into the CTV-E), while LNLs below the threshold are shown in gray (excluded from treatment)}
\label{fig:Treatment_Protocols_N+_II_III}
\end{figure}

% TREATMENT GUIDELINES FOR N+ Ipsilateral LNL II + Contralateral II

\begin{figure}[H]
\centering
\scriptsize

\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Current Clinical Practice (DAHANCA)}
    \label{fig:Treatment_Protocols_N+_II_II_Clinical}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_Clinical_Protocol_N+_II_II.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Clinical_Protocol_N+_II_II.png}
    \end{minipage}
    
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 2\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_II_2}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_2_procent_N+_II_II.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_2_procent_N+_II_II.png}
    \end{minipage}
    
\end{subfigure}

\vspace{1mm}

\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 5\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_II_5}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_5_procent_N+_II_II.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_5_procent_N+_II_II.png}
    \end{minipage}
    
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 8\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_II_8}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_8_procent_N+_II_II.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_8_procent_N+_II_II.png}
    \end{minipage}
    
\end{subfigure}

\vspace{1mm}

\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 10\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_II_10}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_10_procent_N+_II_II.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_10_procent_N+_II_II.png}
    \end{minipage}
    
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 12\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_II_12}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_12_procent_N+_II_II.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_12_procent_N+_II_II.png}
    \end{minipage}
    
\end{subfigure}

\vspace{1mm}

\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 15\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_II_15}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_15_procent_N+_II_II.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_15_procent_N+_II_II.png}
    \end{minipage}
    
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
    \centering
    \caption{Model-based for 20\% Risk Threshold}
    \label{fig:Treatment_Protocols_N+_II_II_20}
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Ipsilateral_model_Protocol_20_procent_N+_II_II.png}
    \end{minipage}%
    \begin{minipage}{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/New_treatment_Protocols/Contralateral_Model_Protocol_20_procent_N+_II_II.png}
    \end{minipage}
    
\end{subfigure}

\caption{Estimated elective nodal irradiation strategies for a patient with an advanced-stage central oropharyngeal tumour and N+ disease in ipsilateral and contralateral LNL II under varying risk thresholds. LNLs above the inclusion threshold are shown in orange (included into the CTV-E), while LNLs below the threshold are shown in gray (excluded from treatment)}
\label{fig:Treatment_Protocols_N+_II_II}
\end{figure}

==> tables.tex <==
% %%%%%%%%%%%%%%%%%%% BELOW HERE IS THE TABLE FOR PATIENT CHARACTERISTICS %%%%%%%%%%%%%%%%%%%
\begin{table}[H]
\centering
\caption{Patient characteristics of retrospective included patients (N = 428)}
\label{tab:baseline_char}
\begin{tabular}{llcc}
\toprule
\textbf{Characteristic} & \textbf{Category} & \textbf{N} & \textbf{\%} \\
\midrule
\textbf{Sex} \\
\hspace{3mm} & Male   & 309 & 72.2 \\
\hspace{3mm} & Female & 119 & 27.8 \\
\addlinespace
\textbf{Primary Tumor Origin} \\
\hspace{3mm} & Base of tongue            & 141 & 33.0 \\
\hspace{3mm} & Vallecula                 & 23  & 5.4  \\
\hspace{3mm} & Tonsil                    & 170 & 39.7 \\
\hspace{3mm} & Pharyngeal arches/Tonsillar fossa & 57 & 13.3 \\
\hspace{3mm} & Glossotonsillar sulcus    & 7   & 1.6  \\
\hspace{3mm} & Posterior pharyngeal wall & 12  & 2.8  \\
\hspace{3mm} & Inferior soft palate      & 13  & 3.0  \\
\hspace{3mm} & Uvula                     & 5   & 1.2  \\
\addlinespace
\textbf{T97 Classification} \\
\hspace{3mm} & T1    & 104 & 24.3 \\
\hspace{3mm} & T2    & 171 & 40.0 \\
\hspace{3mm} & T3    & 89  & 20.8 \\
\hspace{3mm} & T4    & 64  & 14.9  \\
\addlinespace
\textbf{T-Stage Stratification} \\
\hspace{3mm} & Early (T1/T2)          & 275 & 64.7 \\
\hspace{3mm} & Advanced (T3/T4)   & 153 & 35.3 \\
\bottomrule
\end{tabular}
\end{table}


% %%%%%%%%%%%%%%%%%%% BELOW HERE IS THE TABLE FOR SAMPLE PARAMS %%%%%%%%%%%%%%%%%%%

\begin{table}[H]
\centering
\begin{threeparttable}
\caption{The Monte Carlo Markov Chain sampling configurations with the retained sample count}
\label{tab:sampling_config}
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{6pt}
\sisetup{group-separator = {\,}, group-minimum-digits = 4} % local to this table
\begin{tabularx}{\textwidth}{@{}l l X@{}}
\toprule
\textbf{Setting} & \textbf{Value} & \textbf{Notes} \\
\midrule
Number of walkers & $500$ & Parallel, connected ensemble of Markov chains (“walkers”). \\
Steps per walker  & $9000$   & Total steps generated per walker. \\
Initialization    & $\mathcal{U}([0,1]^d)$ & Each walker initialized at a random position drawn uniformly. \\
Proposal mixture (DE/Snooker)  & 80\% \,/\, 20\%  & Differential–evolution moves and snooker updates to efficiently traverse the parameter space while remaining robust to affine transformations. \\
Burn-in (steps per walker)        & 6000  & First \num{6000} steps of each chain discarded. \\
Retained per walker (steps) & 3000  & Used to form the posterior sample set. \\
\addlinespace[2pt]
\textbf{Total retained samples} & \(\num{3000} \times \num{500} = \num{1500000}\) & Posterior sample set size after burn-in removal. \\
\bottomrule
\end{tabularx}
\begin{tablenotes}
\footnotesize
\item $\mathcal{U}([0,1]^d)$: uniform distribution on the $d$-dimensional unit hypercube. DE: differential–evolution move; “snooker”: snooker update (See \cite{nelson_run_2013, ter_braak_differential_2008} for details).
\end{tablenotes}
\end{threeparttable}
\end{table}



% %%%%%%%%%%%%%%%%%%% BELOW HERE IS THE TABLE FOR BN PARAMS %%%%%%%%%%%%%%%%%%%

\begin{table}[H]
\centering
\begin{threeparttable}
\caption{Posterior medians with asymmetric bounds for transition ($\mathrm{t}$) and base ($\mathrm{b}$) proabilities. 
$\mathrm{X}^{\mathrm{i}/\mathrm{c}}_{\mathrm{I\text{--}IV}}$ denote ipsilateral/contralateral LNLs I–IV, and $\mathrm{T}$ is the primary tumour. Bounds reflect the reported asymmetric credible intervals.}
\label{tab:BN_Params}
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{5.5pt}
\begin{tabularx}{\textwidth}{@{}L
S[table-format=1.4] S[table-format=1.4]@{\text{-} \,}S[table-format=1.4]
S[table-format=1.4] S[table-format=1.4]@{\text{-} \,}S[table-format=1.4]@{}}
\toprule
& \multicolumn{3}{c}{Early-stage} & \multicolumn{3}{c}{Advanced-stage} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Arcs & {Median (\%)} & \multicolumn{2}{c}{Bounds (\%)} & {Median (\%)} & \multicolumn{2}{c}{Bounds (\%)} \\
\midrule

\multicolumn{7}{@{}l}{\textbf{Ipsilateral Transition Probabilities} ($\mathrm{t}^{\mathrm{i}}$)}\\
\addlinespace[2pt]
$\mathrm{X}^{\mathrm{i}}_{\mathrm{I}}\!\to\!\mathrm{X}^{\mathrm{i}}_{\mathrm{II}} \; (\mathrm{t}^{\mathrm{i}}_{1,2})$
  & 0.200 & 0.060 & 0.400 & 0.170 & 0.050 & 0.360 \\
$\mathrm{X}^{\mathrm{i}}_{\mathrm{II}}\!\to\!\mathrm{X}^{\mathrm{i}}_{\mathrm{III}} \; (\mathrm{t}^{\mathrm{i}}_{2,3})$
  & 0.350 & 0.310 & 0.390 & 0.430 & 0.370 & 0.480 \\
$\mathrm{X}^{\mathrm{i}}_{\mathrm{III}}\!\to\!\mathrm{X}^{\mathrm{i}}_{\mathrm{IV}} \; (\mathrm{t}^{\mathrm{i}}_{3,4})$
  & 0.200 & 0.160 & 0.240 & 0.180 & 0.130 & 0.230 \\

\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textbf{Ipsilateral Base Probabilities} ($\mathrm{b}^{\mathrm{i}}$)}\\
\addlinespace[2pt]
$\mathrm{T}\!\to\!\mathrm{X}^{\mathrm{i}}_{\mathrm{I}} \; (\mathrm{b}^{\mathrm{i}}_{1})$
  & 0.035 & 0.026 & 0.045 & 0.120 & 0.100 & 0.150 \\
$\mathrm{T}\!\to\!\mathrm{X}^{\mathrm{i}}_{\mathrm{II}} \; (\mathrm{b}^{\mathrm{i}}_{2})$
  & 0.790 & 0.770 & 0.810 & 0.860 & 0.830 & 0.880 \\
$\mathrm{T}\!\to\!\mathrm{X}^{\mathrm{i}}_{\mathrm{III}} \; (\mathrm{b}^{\mathrm{i}}_{3})$
  & 0.063 & 0.043 & 0.093 & 0.075 & 0.035 & 0.135 \\
$\mathrm{T}\!\to\!\mathrm{X}^{\mathrm{i}}_{\mathrm{IV}} \; (\mathrm{b}^{\mathrm{i}}_{4})$
  & 0.009 & 0.004 & 0.015 & 0.029 & 0.019 & 0.049 \\

\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textbf{Contralateral Transition Probabilities} ($\mathrm{t}^{\mathrm{c}}$)}\\
\addlinespace[2pt]
$\mathrm{X}^{\mathrm{c}}_{\mathrm{I}}\!\to\!\mathrm{X}^{\mathrm{c}}_{\mathrm{II}} \; (\mathrm{t}^{\mathrm{c}}_{1,2})$
  & 0.270 & 0.080 & 0.550 & 0.270 & 0.080 & 0.550 \\
$\mathrm{X}^{\mathrm{c}}_{\mathrm{II}}\!\to\!\mathrm{X}^{\mathrm{c}}_{\mathrm{III}} \; (\mathrm{t}^{\mathrm{c}}_{2,3})$
  & 0.200 & 0.150 & 0.260 & 0.230 & 0.180 & 0.280 \\
$\mathrm{X}^{\mathrm{c}}_{\mathrm{III}}\!\to\!\mathrm{X}^{\mathrm{c}}_{\mathrm{IV}} \; (\mathrm{t}^{\mathrm{c}}_{3,4})$
  & 0.230 & 0.130 & 0.350 & 0.330 & 0.240 & 0.420 \\

\addlinespace[2pt]
\multicolumn{7}{@{}l}{\textbf{Contralateral Base Probabilities} ($\mathrm{b}^{\mathrm{c}}$)}\\
\addlinespace[2pt]
$\mathrm{T}\!\to\!\mathrm{X}^{\mathrm{c}}_{\mathrm{I}} \; (\mathrm{b}^{\mathrm{c}}_{1})$
  & 0.006 & 0.001 & 0.009 & 0.010 & 0.004 & 0.018 \\
$\mathrm{T}\!\to\!\mathrm{X}^{\mathrm{c}}_{\mathrm{II}} \; (\mathrm{b}^{\mathrm{c}}_{2})$
  & 0.140 & 0.120 & 0.160 & 0.450 & 0.410 & 0.490 \\
$\mathrm{T}\!\to\!\mathrm{X}^{\mathrm{c}}_{\mathrm{III}} \; (\mathrm{b}^{\mathrm{c}}_{3})$
  & 0.010 & 0.005 & 0.015 & 0.040 & 0.020 & 0.060 \\
$\mathrm{T}\!\to\!\mathrm{X}^{\mathrm{c}}_{\mathrm{IV}} \; (\mathrm{b}^{\mathrm{c}}_{4})$
  & 0.002 & 0.000 & 0.005 & 0.010 & 0.003 & 0.020 \\

\bottomrule
\end{tabularx}
\begin{tablenotes}
\footnotesize
\item \emph{Note:} Values are reported as median and bounds \([\,\text{lower},\,\text{upper}\,]\) derived from the original asymmetric uncertainties \(x^{+u}_{-l}\) (lower \(= x-l\), upper \(= x+u\)).
\end{tablenotes}
\end{threeparttable}
\end{table}







% %%%%%%%%%%%%%%%%%%% BELOW HERE IS THE TABLE FOR RESULTS %%%%%%%%%%%%%%%%%%%


% Please add the following required packages to your document preamble:
% \begin{table}[H]
% \centering
% \begin{tabular}{cc|cccc|}
% \cline{3-6}
% \multicolumn{1}{l}{}                                                              &                       & \multicolumn{4}{c|}{\multirow{2}{*}{\textbf{Risk of Involvement(\%)}}}                                                               \\
% \multicolumn{1}{l}{}                                                              & \multicolumn{1}{l|}{} & \multicolumn{4}{c|}{}                                                                                                    \\
% \multicolumn{1}{l}{}                                                              &                       & \textbf{I}                     & \textbf{II}                    & \textbf{III}                   & \textbf{IV}           \\ \hline
% \multicolumn{1}{|c}{\multirow{6}{*}{\textbf{Observed Ipsilateral Involvement}}}   & \textbf{I}            & \multicolumn{1}{c|}{\rule[0.5ex]{1em}{0.6pt}} & \multicolumn{1}{c|}{47.9/\textbf{56.3}} & \multicolumn{1}{c|}{7.8/\textbf{11.0}}   & $< 1.0$/\textbf{1.4}           \\
% \multicolumn{1}{|c}{}                                                             & \textbf{II}           & \multicolumn{1}{c|}{$< 1.0$/\textbf{3.9}}   & \multicolumn{1}{c|}{\rule[0.5ex]{1em}{0.6pt}} & \multicolumn{1}{c|}{13.5/\textbf{21.6}} & 1.2/\textbf{2.3}               \\
% \multicolumn{1}{|c}{}                                                             & \textbf{II+III}       & \multicolumn{1}{c|}{$< 1.0$/\textbf{3.1}}   & \multicolumn{1}{c|}{\rule[0.5ex]{1em}{0.6pt}} & \multicolumn{1}{c|}{\rule[0.5ex]{1em}{0.6pt}} & 4.3/\textbf{4.4}               \\
% \multicolumn{1}{|c}{}                                                             & \textbf{III}          & \multicolumn{1}{c|}{1.3/\textbf{4.6}}   & \multicolumn{1}{c|}{76.0/\textbf{82.6}} & \multicolumn{1}{c|}{\rule[0.5ex]{1em}{0.6pt}} & 4.3/\textbf{8.3}              \\
% \multicolumn{1}{|c}{}                                                             & \textbf{IV}           & \multicolumn{1}{c|}{1.0/\textbf{4.8}}          & \multicolumn{1}{c|}{45.4/\textbf{63.5}}          & \multicolumn{1}{c|}{16.8/\textbf{22.3}}          & \multicolumn{1}{c|}{\rule[0.5ex]{1em}{0.6pt}} \\
% \multicolumn{1}{|c}{}                                                             & \textbf{N0}           & \multicolumn{1}{c|}{1.3/\textbf{3.3}}   & \multicolumn{1}{c|}{48.6/\textbf{60.4}} & \multicolumn{1}{c|}{8.9/\textbf{13.3}}   & $< 1.0$/\textbf{1.6}               \\ \hline
% \multicolumn{1}{|c}{\multirow{6}{*}{\textbf{Observed Contralateral Involvement}}} & \textbf{I}            & \multicolumn{1}{c|}{\rule[0.5ex]{1em}{0.6pt}}  & \multicolumn{1}{c|}{5.3/\textbf{20.1}}   & \multicolumn{1}{c|}{$< 1.0$/\textbf{3.3}}   & $< 1.0$/$\mathbf{< 1.0}$               \\
% \multicolumn{1}{|c}{}                                                             & \textbf{II}           & \multicolumn{1}{c|}{$< 1.0$/$\mathbf{< 1.0}$}   & \multicolumn{1}{c|}{\rule[0.5ex]{1em}{0.6pt}} & \multicolumn{1}{c|}{4.2/\textbf{7.1}}   & $< 1.0$/\textbf{1.8}               \\
% \multicolumn{1}{|c}{}                                                             & \textbf{II+III}       & \multicolumn{1}{c|}{$< 1.0$/$\mathbf{< 1.0}$ }   & \multicolumn{1}{c|}{\rule[0.5ex]{1em}{0.6pt}} & \multicolumn{1}{c|}{\rule[0.5ex]{1em}{0.6pt}} & 4.2\textbf{/6.9}               \\
% \multicolumn{1}{|c}{}                                                             & \textbf{III}          & \multicolumn{1}{c|}{$< 1.0$/$\mathbf{< 1.0}$ }   & \multicolumn{1}{c|}{9.4/\textbf{38.4}}  & \multicolumn{1}{c|}{\rule[0.5ex]{1em}{0.6pt}}  & $< 1.0$/\textbf{2.4}               \\
% \multicolumn{1}{|c}{}                                                             & \textbf{IV}           & \multicolumn{1}{c|}{$< 1.0$/$\mathbf{< 1.0}$ }          & \multicolumn{1}{c|}{4.7/\textbf{19.1}}          & \multicolumn{1}{c|}{1.2/\textbf{7.5}}          & \multicolumn{1}{c|}{\rule[0.5ex]{1em}{0.6pt}} \\
% \multicolumn{1}{|c}{}                                                             & \textbf{N0}           & \multicolumn{1}{c|}{$< 1.0$/$\mathbf{< 1.0}$ }   & \multicolumn{1}{c|}{3.9/\textbf{18.1}}   & \multicolumn{1}{c|}{$< 1.0$/\textbf{2.8}}   & $< 1.0$/$\mathbf{< 1.0}$            \\ \hline
% \end{tabular}
% \caption{Probabilities of harbouring nodal involvement in each lymph node level (LNL), conditional on the observed (radiologically apparent) involvement pattern on diagnostic imaging. Each row represents a specific observed pattern of involved LNLs, while each column indicates the predicted risk (\%) of true nodal involvement in the respective LNL, as computed according to equation \ref{eq:computing_risk}. Probabilities reported in bold correspond to predictions for advanced-stage tumours. The hyphen ("\rule[0.5ex]{1em}{0.6pt}") indicates that, if a given LNL is observed as involved on diagnostic imaging, it is assumed by default that this level will be included in the elective target volume, thus, the risk is not computed or reported for these LNLs.}
% \label{tab:Results}
% \end{table}
